Learning Perception-Aware Agile Flight in Cluttered Environments

Recently, neural control policies have outperformed existing model-based planning-and-control methods for autonomously navigating quadrotors through cluttered environments in minimum time. However, they are not perception aware, a crucial requirement in vision-based navigation due to the camera's limited field of view and the underactuated nature of a quadrotor. We propose a learning-based system that achieves perception-aware, agile flight in cluttered environments. Our method combines imitation learning with reinforcement learning (RL) by leveraging a privileged learning-by-cheating framework. Using RL, we first train a perception-aware teacher policy with full-state information to fly in minimum time through cluttered environments. Then, we use imitation learning to distill its knowledge into a vision-based student policy that only perceives the environment via a camera. Our approach tightly couples perception and control, showing a significant advantage in computation speed (10 times faster) and success rate. We demonstrate the closed-loop control performance using hardware-in-the-loop simulation.

==> tables/obs_new.tex <==
\begin{table*}[htp]
\renewcommand\arraystretch{1.2}
\renewcommand{\tabcolsep}{6.4pt} 
\centering
\caption{Comparison between the baseline algorithm~\cite{penicka2022minimum}  and the proposed state-based and vision-based policies in non- and perception-aware mode. \label{tab:state_vision_new}}
% \begin{spacing}{1.2}
\begin{tabular}{lccccccccc}
\hline
\multirow{4}*{\textbf{Environment}} & \multirow{4}*{\textbf{Case}} & 
\multicolumn{4}{c}{\textbf{Non-perception-aware}} & \multicolumn{4}{c}{\textbf{Perception-aware (ours)}}\\
\cmidrule(lr){3-6} \cmidrule(lr){7-10}
& & \multicolumn{2}{c}{\textbf{Sampling-based + MPC}} & \multicolumn{2}{c}{\textbf{State-based}} & \multicolumn{2}{c}{\textbf{State-based (teacher)}} & \multicolumn{2}{c}{\textbf{Vision-based (student)}}  \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} %\\[-1em]
                        &   & Success[\%] & Time[s] & Success[\%] & Time[s] & Success[\%] & Time[s]     & Success[\%]      & Time[s] \\
\hline
\multirow{4}*{Columns}   & 0 & 25 & 1.22     & 100        & \textbf{1.10$\pm$0.02} & 100        & 1.16$\pm$0.02        & 100      & \textbf{1.10$\pm$0.02} \\
                        & 1 & 0 & -         & 100        & \textbf{1.10$\pm$0.02} & 100        & \textbf{1.10$\pm$0.03}        & 100      & \textbf{1.10$\pm$0.03} \\
                        & 2 & 27 & 1.14     & 100        & \textbf{1.10$\pm$0.02} & 100        & \textbf{1.10$\pm$0.02}        & 100      & \textbf{1.10$\pm$0.03} \\
                        & 3 & 16 & 1.70     & 100        & 1.40$\pm$0.04 & 100        & 1.46$\pm$0.04        & 100      & \textbf{1.39$\pm$0.04}  \\
\hline
\multirow{4}*{Office}   & 0 & 41 & 2.38     & 100        & 1.80$\pm$0.04 & 100        & 1.92$\pm$0.04        & 100      & \textbf{1.79$\pm$0.04}  \\
                        & 1 & 28 & 1.86     & 100        & 1.80$\pm$0.03 & 100        & 1.82$\pm$0.02        & 100      & \textbf{1.76$\pm$0.02}  \\
                        & 2 & 56 & 2.29     & 100        & \textbf{1.62$\pm$0.02} & 100        & 1.66$\pm$0.03        & 100      & 1.63$\pm$0.03  \\
                        & 3 & 70 & 2.16     & 100        & 1.46$\pm$0.02 & 100        & 1.48$\pm$0.02        & 100      & \textbf{1.45$\pm$0.02}  \\
\hline
\multirow{4}*{Racing}   & 0 & 57 & 1.61     & 100        & 1.33$\pm$0.03 & 100        & \textbf{1.32$\pm$0.02}        & 100      & 1.33$\pm$0.03  \\
                        & 1 & 51 & 1.64     & 100        & \textbf{1.30$\pm$0.02} & 100        & 1.42$\pm$0.03        & 100      & 1.31$\pm$0.04  \\
                        & 2 & 76 & 1.72     & 100        & \textbf{1.42$\pm$0.02} & 100        & 1.44$\pm$0.02        & 100      & 1.43$\pm$0.02  \\
                        & 3 & 54 & 1.80     & 100        & 1.42$\pm$0.02 & 100        & 1.48$\pm$0.02        & 100      & \textbf{1.39$\pm$0.01}  \\
\hline
Racing MW             & 0 & 25 & 7.22       & 100        & \textbf{7.78$\pm$0.07}  & 100        & 8.52$\pm$0.04        & 100      &  8.34$\pm$0.06\\
% \hline
% Arena                  & 0 & 100        & 7.68$\pm$0.04        & 100      & 8.81$\pm$0.05  \\
\hline
\end{tabular}
% \end{spacing}
% \vspace{0.5mm}
% \robert{I would add non-perception-aware results for comparison, either only Robert's RAL, but rather also the other baselines such as Poly/search-based etc. from Robert's RAL}
% }
\end{table*}

==> tables/obs_sci_perform.tex <==
\begin{table*}[htp]
\centering
% \makeatletter\def\@captype{table}\makeatother
\centering
% \begin{spacing}{1.2}
\begin{tabular}{lcccc}
\toprule
\multirow{2}*{\textbf{Method}} & \multirow{2}*{\textbf{Speed[m/s]}}& {\textbf{Sci Paper}} & \multicolumn{2}{c}{\textbf{Ours}}  \\
                        &   & Success[\%]     & Success[\%]      & Time[s] \\
\hline
\multirow{5}*{Forest}   & 3 & 100               &       &  \\
                        & 5 & 100               &       &  \\
                        & 7 & 90                &       &  \\
                        & 10 & 60               & 100   & 5.56$\pm$0.03  \\
                        % & 40 & -                 & 90   & 2.04$\pm$0.02 \\
\hline
\multirow{5}*{Narrow Gap}   & 1 & 100           &       &   \\
                        & 3 & 100               &       &   \\
                        & 5 & 100               &       &   \\
                        & 7 & 80                & 100   & 8.04$\pm$0.02  \\
                        % & 40 & -                 & 100   & 2.12$\pm$0.02 \\
\bottomrule
\end{tabular}
\caption{Baseline Comparisons \robert{I would not add the Forest with Walls row because we do not have results for sci paper for it and we can not say like in the last rows of other environments that it is bacues they are not capable of it....}}
\end{table*}
